CoKe: Customizable Fine-Grained Story Evaluation via Chain-of-Keyword Rationalization

Evaluating creative text such as human-written stories using language models has always been a challenging task -- owing to the subjectivity of multi-annotator ratings. To mimic the thinking process of humans, chain of thought (CoT) generates free-text explanations that help guide a model's predictions and Self-Consistency (SC) marginalizes predictions over multiple generated explanations. In this study, we discover that the widely-used self-consistency reasoning methods cause suboptimal results due to an objective mismatch between generating 'fluent-looking' explanations vs. actually leading to a good rating prediction for an aspect of a story. To overcome this challenge, we propose $\textbf{C}$hain-$\textbf{o}$f-$\textbf{Ke}$ywords (CoKe), that generates a sequence of keywords $\textit{before}$ generating a free-text rationale, that guide the rating prediction of our evaluation language model. Then, we generate a diverse set of such keywords, and aggregate the scores corresponding to these generations. On the StoryER dataset, CoKe based on our small fine-tuned evaluation models not only reach human-level performance and significantly outperform GPT-4 with a 2x boost in correlation with human annotators, but also requires drastically less number of parameters.

==> sections/preliminaries_old.tex <==
\section{Problem Formulation}
\label{sec:formulation}

\brihi{Describe Figure 1 and Evaluation}

We begin by describing our task setup, our evaluation scheme and the dataset that we use for all of our experiments. 
\autoref{fig:pitch_figure} describes our formulation and task.
\brihi{Edit intro line for this section}

\paragraph{Task Setup.} We are given a story with an arbitrary length, along with an aspect, with respect to which we view the story. 
The aspect by itself can be arbitrary as well, which can focus on certain semantic or literary features of the story \brihi{cite}, like \textit{humor}, \textit{character shaping}, etc.
Our task is to evaluate the story with respect to the aspect given, and provide a floating-point score, normalized to be between $0$ and $1$, where a higher score implies that the aspect is well incorporated in the story.
However, along with the score, we also want to generate an \textit{explanation} that can reason `why' the given score was allotted to an aspect-story pair. 

% \paragraph{Task Setup.} We are given a story with an arbitrary length, along with an aspect, with respect to which we wish to evaluate the story. 
% The aspect by itself can be arbitrary as well.
% An evaluation system will provide us with a floating-point score, normalized to be between $0$ and $1$, where a higher score implies that the aspect is well incorporated in the story.
% Along with a score, it will also provide an `explanation' that can reason `why' a given score was allotted to an aspedt-story pair.

\paragraph{Evaluation Scheme.} 

\brihi{Mention normalization in 0-1}

We assume two real-world constraints in our evaluation scheme. \brihi{cite}
Firstly, any automated story evaluation system would only be able to provide a single score for an aspect-story pair, without modelling the annotator itself \brihi{cite annotator identities paper}. 
Secondly, while an automated system can only provide a single score, there can be multiple human annotators that can subjectively evaluate the story.
Our evaluation scheme considers these two constraints by comparing any automated story evaluation system's scores with all the human annotators separately (without any aggregation of human scores), so as to align it as closely as possible to different annotators.
We report three metrics for every evaluation conducted -- Pearson's Correlation Coefficient (PCC), Mean Squared Error (MSE) and F1-score on binarized score values. 

\paragraph{Story evaluation is an extremely subjective task. }

We use the StoryER dataset \citep{chen-etal-2022-storyer} as a pilot dataset for our task.
The StoryER dataset extends the WritingPrompts \citep{fan-etal-2018-hierarchical} dataset, which consists of multiple writing prompts and corresponding human-written stories for those prompts, by adding ratings for ten \textit{aspects} that are picked by the authors from a given list of fixed aspects, along with \textit{comments} that justify the corresponding ratings given. 

\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-12pt}
  \begin{center}
    \includegraphics[width=0.48\textwidth]{figures/annotator_agreement.pdf}
  \end{center}
  \caption{Annotator Agreements for different aspects. \brihi{Placeholder image for annotator agreements}}
  \label{fig:annotator_agreements}
  \vspace{-12pt}
\end{wrapfigure}

Each of these aspects aims to highlight a separate semantic or literal aspect of the story -- for example, aspects can highlight the `ending' or `humour'-level of a story.
This is done by multiple annotators for every writing prompt + story pair, however the number of annotators, and actual aspects (out of ten) that are annotated for a story can vary.
\brihi{A description of these aspects, along with statistics of the dataset is given in Table \ref{Add Table}.\brihi{Add table}}

What is interesting to note here is that human evaluations with respect to the these aspects are extremely subjective.
We calculate Intraclass Correlation Coefficient (ICC) scores \citep{iccscore} to evaluate annotator agreements within annotators for a given aspect, across all the possible stories which are marked with that aspect (\autoref{fig:annotator_agreements}).
The `heartwarming' aspect has the highest agreement of $0.37$, which is still considered to be poor while interpreting ICC scores \citep{iccscore}.

Another demonstration of this subjectivity is while calculating \textsc{Human Performance} scores from the dataset.
In order to calculate human performance, we randomly select a score from one annotator, and use that as a prediction to estimate other annotators, which better represents the setting that automated story evaluation systems would fall into (assume the prediction from the system to be one `annotator' that tries to best approximate other annotators). \brihi{should we add a line about the human performance score from the main table here?}

\paragraph{Subjectivity arises due to annotator artifacts.}
\label{sec:subjectivity}

\brihi{Modify paragraph to the storyline that we discussed}


\brihi{Table \brihi{Add Table} shows examples of annotator \textit{justifications} provided for rating a story for the same aspect.}
As we note earlier that the annotator scores are subjective, looking into these justifications demonstrates that different annotators have different artifacts they rely on for decision making \brihi{cite}.
We can see that annotators use certain sentiment-laden phrases (\textit{i love this!, this is pathetic}, etc), have different knowledge priors (\textit{it could be better explained., this is too much detail we all know what it is}, etc) or focus on different components of the story to evaluate the same aspect (\textit{I did like the back-and-forth questioning between the attorney and God, score: 0.75} v.s. \textit{The description was totally a mess and it didn't have any emotion. It was just soulless and was totally bad., score: 0.0}). \brihi{ending line?}
\brihi{Replace inline examples with highlighted table}

% the dataset contains significant annotator disagreement -- the highest annotator agreement (within annotators, across different stories) is $0.37$ for the `heartwarming' aspect, which is still considered poor agreement. \brihi{Add citation from wiki}

% \begin{figure*}[t!]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.2in]{figures/annotator_agreement.pdf}
%         \caption{Lorem ipsum}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[height=1.2in]{figures/human_upper_bounds.png}
%         \caption{Lorem ipsum, lorem ipsum,Lorem ipsum, lorem ipsum,Lorem ipsum}
%     \end{subfigure}
%     \caption{Caption place holder}
% \end{figure*}

% \paragraph{Human Performance. } 
% We then calculate different variants of human performance that is estimated from the multiple-annotator annotations that the StoryER test set contains.
% \brihi{Find references in existing literature for these variants}
% \autoref{fig:human_perf} contains a visual description of these variants.
% Optimal Prediction and Majority Voting includes taking the mean and mode of the annotator predictions respectively as predictions.
% However, they work under the assumption that ratings of all annotators are available at test time, which is not a realistic setting.
% The Human Predicting Human variant randomly selects a rating from one annotator, and uses that as a prediction to estimate other annotators, which better represents the setting that our evaluation systems would fall into (assume the prediction from the system to be one `annotator' that tries to best approximate other annotators).
% \brihi{Add one line inference from the table}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.9\textwidth]{figures/human_upper_bounds.png}
%     \caption{\brihi{Placeholder figure for human upper bound calculation}}
%     \label{fig:human_perf}
% \end{figure}
